Smart Environment for Adaptive Learning of Cybersecurity Skills

Hands-on computing education requires a realistic learning environment that enables students to gain and deepen their skills. Available learning environments, including virtual and physical labs, provide students with real-world computer systems but rarely adapt the learning environment to individual students of various proficiency and background. We designed a unique and novel smart environment for adaptive training of cybersecurity skills. The environment collects a variety of student data to assign a suitable learning path through the training. To enable such adaptiveness, we proposed, developed, and deployed a new tutor model and a training format. We evaluated the learning environment using two different adaptive trainings attended by 114 students of various proficiency. The results show students were assigned tasks with a more appropriate difficulty, which enabled them to successfully complete the training. Students reported that they enjoyed the training, felt the training difficulty was appropriately designed, and would attend more training sessions like these. Instructors can use the environment for teaching any topic involving real-world computer networks and systems because it is not tailored to particular training. We freely released the software along with exemplary training so that other instructors can adopt the innovations in their teaching practice.

==> figures/post-training-questionnaire.tex <==
\begin{table}[h!]
    \centering
    \caption{Wording of the post-training questionnaire.}
    \label{tab:postGameAssessmentQuestions}
    \small
    \begin{tabular}{p{0.3cm}|p{7.3cm}}
    \hline 
    \textbf{No.} & \textbf{Question} \\  \hline
        Q1 & Did you feel the tasks were designed so that you can complete the training in a timely manner?  \\ 
        Q2 & Did you feel you got stuck at some point during the training?  \\ 
        Q3 & How much did you enjoy the training?  \\
        Q4 & Did you feel the training should be more difficult for you?  \\
        Q5 & Did you feel you would like the training to be longer with additional tasks to solve?  \\
        Q6 & Would you like to play more cybersecurity training sessions like this one?  \\
        \hline
    \end{tabular}
\end{table}

